Open-Vocabulary 3D Semantic Segmentation with Text-to-Image Diffusion Models

In this paper, we investigate the use of diffusion models which are pre-trained on large-scale image-caption pairs for open-vocabulary 3D semantic understanding. We propose a novel method, namely Diff2Scene, which leverages frozen representations from text-image generative models, along with salient-aware and geometric-aware masks, for open-vocabulary 3D semantic segmentation and visual grounding tasks. Diff2Scene gets rid of any labeled 3D data and effectively identifies objects, appearances, materials, locations and their compositions in 3D scenes. We show that it outperforms competitive baselines and achieves significant improvements over state-of-the-art methods. In particular, Diff2Scene improves the state-of-the-art method on ScanNet200 by 12%.

==> tables/exp_nr3d_main.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
    \toprule
    Method              & K=\# distractors   & K=10 & K=15 \\
    \midrule
    
    OpenScene (2D, OS) \cite{openscene} & 79.1    & 20.0    & 12.4          \\
    OpenScene (3D, OS)  \cite{openscene}       & 74.3    & 19.1     & 13.3          \\
    OpenScene (2D/3D, OS)  \cite{openscene}         & 72.4    &  21.0  & 14.3         \\
    \textbf{Diff2Scene (Ours)}    & \textbf{81.9}     & \textbf{22.9}    & \textbf{17.1}      \\
   
    \bottomrule
\end{tabular}
% }
\caption{\textbf{Comparison with OpenScene \cite{openscene} on visual grounding dataset Nr3D.} Following \cite{achlioptas2020referit_3d}, we match the predicted mask and $K$ ground truth masks and use the matching accuracy as the evaluation metric. We set $K$ to be the number of distractors (the objects in the same category of the referred object), and two fixed number 10 and 15. We observe that our method significantly outperforms OpenScene in all experimental setups.}
\label{table:nr3d}
\end{table}
